Multipolar gravitational waveforms for spinning binary black holes and their impact on source characterization

In the last five years, gravitational-wave astronomy has gone from a purely theoretical field into a thriving experimental science. Many gravitational-wave signals, emitted by stellar-mass binary black holes and binary neutron stars, have been detected, and many more are expected in the future. The observation of the gravitational-wave signals from these systems, and the characterization of their sources, heavily relies on the precise models for the emitted gravitational waveforms. In this thesis, I present an updated version of the waveform models for spinning binary black holes within the effective-one-body formalism. The novelty of the waveform models presented in this work is the inclusion of beyond-quadupolar terms in the waveforms emitted by spinning binary black holes. I first construct the model in the simplified case of black holes with spins aligned with the orbital angular momentum of the binary, then I extend it to the case of generic spin orientations. The measurement of the source properties of a binary system emitting gravitational waves requires to compute $\mathcal{O}(10^7-10^9)$ different waveforms. Since the waveform models mentioned before can require $\mathcal{O}(1-10)$s to generate a single waveform, they can be difficult to use in data-analysis studies. To overcome this obstacle, I use the reduced-order-modeling technique to develop a faster version of the waveform model for black holes with spins aligned to the orbital angular momentum of the binary. The waveform models developed in this thesis have been used by the LIGO and Virgo collaborations for the inference of the source parameters of the gravitational-wave signals detected during the second and third observing runs (O2 and O3) of the LIGO and Virgo detectors. Here, I present a study on the source properties of the signals GW170729 and GW190412, for which I have been directly involved in the analysis.

==> etc/acronym.tex <==
%******************************************************
%*    LaTex-Vorlage für wissenschaftliche Arbeiten    *
%*    --------------------------------------------    *
%*      Autor: Jan Brennenstuhl (@jbspeakr)           *
%*             www.funkblocka.de                      *
%*            Lizenz: CC BY-SA 3.0                    *
%******************************************************
\newacronym[\glslongpluralkey={Public-Key-Infrasturkturen}]{PKI}{PKI}{Public-Key-Infrasturktur}
\newacronym{IDM}{IDM}{Identity-Management}
\newacronym{ESB}{ESB}{Enterprise-Service-Bus}
\newacronym{ID}{ID}{Identifikator} 
\newacronym{SigG}{SigG}{Signaturgesetz}
\newacronym{CCC}{CCC}{Chaos Computer Club e. V.}
\newacronym{BSI}{BSI}{Bundesamt für Sicherheit in der Informationstechnik}

==> etc/glossary.tex <==
%******************************************************
%*    LaTex-Vorlage für wissenschaftliche Arbeiten    *
%*    --------------------------------------------    *
%*      Autor: Jan Brennenstuhl (@jbspeakr)           *
%*             www.funkblocka.de                      *
%*            Lizenz: CC BY-SA 3.0                    *
%******************************************************
\newglossaryentry{glos:PKI}{
name=Public-Key-Infrasturktur,
description={Eine Public-Key-Infrasturktur ist eine...}
}
\newglossaryentry{glos:SC}{
name=Smart-Card,
description={EineSmart-Card ist eine...}
}
\newglossaryentry{glos:SigG}{
name=Signaturgesetz,
description={EineSmart-Card ist eine...}
}

==> intro/introduction.tex <==
%******************************************************
%*    LaTex-Vorlage für wissenschaftliche Arbeiten    *
%*    --------------------------------------------    *
%*      Autor: Jan Brennenstuhl (@jbspeakr)           *
%*             www.funkblocka.de                      *
%*            Lizenz: CC BY-SA 3.0                    *
%******************************************************
\begin{large}

\vspace*{2cm}
\noindent
Ich versichere, dass ich die von mir vorgelegte Arbeit selbstständig verfasst habe, dass ich die verwendeten Quellen, Internet-Quellen und Hilfsmittel vollständig angegeben habe und dass ich die Stellen der Arbeit - einschließlich Tabellen, Karten und Abbildungen -, die anderen Werken oder dem Internet im Wortlaut oder dem Sinn nach entnommen sind, in jedem Fall unter Angabe der Quelle als Entlehnung kenntlich gemacht habe.\vspace{2cm}

\noindent
Berlin, den 1. Januar 1970

\vspace{3cm}

\hspace*{6cm}%
\dotfill\\
\hspace*{7cm}%
\textit{(Unterschrift des Kandidaten)}

\end{large}


==> sections/1_1-papers_interlude.tex <==
\chapter{Research overview}
\label{chap:res_overview}

Each chapter below is a paper published in an international peer-reviewed journal. Here I briefly summarize my contribution to each of these publications.

\endinput 

==> sections/6-Conclusions_copy.tex <==
\chapter{Conclusions and future work}
\label{chap:six}
The work I have presented in this thesis aimed at improving the models for the \ac{GW} signals emitted by coalescing \acp{BBH} with spins. The accuracy of these waveform models is crucial because they are key components for both the detection and the source characterization of \ac{GW} signals. For this reason, and considering that \ac{GW} detectors are costantly improving their sensitivity, it is important that also the accuracy of waveform models progresses at the same pace.

This thesis revolves around the effect of \acp{HM} in the waveforms emitted by coalescing \acp{BBH} with spins. Their contribution is especially relevant when the total mass of the system is large, there is a big difference between the masses of the two \acp{BH} or the binary system is observed from a direction orthogonal to its angular momentum.

In Chapters 2 and 3 I developed within the \ac{EOB} formalism, inspiral-merger-ringdown waveform models for spinning \acp{BBH} which include \acp{HM}. The waveform model described in Chapter 2, \texttt{SEOBNRv4HM}, is limited to \acp{BH} with spins aligned with the angular momentum of the binary and served as foundation for \texttt{SEOBNRv4PHM}, its generalization to \acp{BH} with generic spin orientations described in Chapter 3.
I tested the accuracy of the waveforms generated with these models by computing the unfaithfulness against about $1700$ \ac{NR} simulations ($\sim 200$ for the first model and $\sim 1500$ for the second one). In the total mass range $20-200\,M_\odot$, \texttt{SEOBNRv4HM} yields average unfaithfulness values smaller than $1\%$ for almost all cases with few exceptions for which the value is slightly above $1\%$. \texttt{SEOBNRv4PHM} is also very accurate and for $94\%$ ($57\%$) of the cases its unfaithfulness against \ac{NR} waveforms is below $3\%$ ($1\%$) in the same mass range. The great accuracy reached by these models is also confirmed by the parameter estimation studies I performed using them to analyze synthetic \ac{GW} signals generated using \ac{NR} waveforms. Both models managed to measure the most relevant binary parameters, such as masses and spins, with negligible bias compared to the statistical uncertainty in binary systems with asymmetric masses, strong precessional effects (in the case of \texttt{SEOBNRv4PHM}) and moderately large values of the \ac{SNR}. \texttt{SEOBNRv4PHM} was even able to unbiasedly recover the parameters of a synthetic \ac{BBH} system for a less extreme binary configuration but at an \ac{SNR} of $50$.

The number of observed \ac{GW} signals steadily increased in the past years and it is expected to rise even more in the next decade as consequence of the upgrades in the \ac{GW} detectors. For this reason, waveform models have to be not only accurate but also fast to timely analyze the increasing number of detected signals. For this reason, in Chapter 3 I developed \texttt{SEOBNRv4HM\_ROM}, a \ac{ROM} version of \texttt{SEOBNRv4HM} which accelerate the generation of the waveforms by two orders of magnitude with negligible loss in the accuracy.

The models I developed in this thesis have been already used in the analysis of \ac{GW} signals detected by the LIGO and Virgo interferometers. In Chapter 4 I present an investigation on the \ac{GW} signal GW170729 performed with waveform models with \acp{HM}, including \texttt{SEOBNRv4HM}. This signal was particularly interesting to study with these waveform models because it was likely originating from the most massive \ac{BBH} system observed during the LIGO and Virgo second observing run. When using \texttt{SEOBNRv4HM} to analyze this signal I obtained improved measurements of the mass ratio and the effective-spin parameter. In particular, the mass ratio measurement allowed to exclude with large confidence that the signal was emitted from a \ac{BBH} with similar masses. In fact, the study with \texttt{SEOBNRv4HM} revealed that with $40\%$ probability the signal was emitted by a \ac{BBH} where the mass of the most massive \ac{BH} in the binary was larger than the mass of the other \ac{BH} by more than a factor of two. This probability was only about $20\%$ when the properties of this signal were measured with waveform models without \acp{HM}. 

As a member of the LIGO Scientific Collaboration I also contributed to the analysis of the \ac{GW} signal GW190412~\cite{LIGOScientific:2020stg} observed during the first half of the third LIGO and Virgo observing run. This signal was interesting to study for the asymmetric masses of its source. In Chapter 1 I summarize the analysis I performed on this system with the waveform models described in the thesis. This investigation confirmed with large confidence that the signal was emitted by a \ac{BBH} with very asymmetric masses. In fact, the median value of $m_1/m_2$ for this system was between $3$ and $5$ and $m_1/m_2 \geq 2$ with a probability of $99\%$. This precise measurement of the mass ratio $m_1/m_2$ allowed to obtain also a tight constraint on the dimensionless spin magnitude of the most massive \ac{BH} in the binary, which value results to be between $0.22$ and $0.60$ at $90 \%$ probability. The luminosity distance was another source property that was very precisely measured in this system because the effect of \acp{HM} and spin precession were present in the waveform models used for the analysis. In fact, the bounds on the luminosity distance resulted to be $\sim 60\%$ tighter compared to those obtained by waveform models without these effects. A precise measurement of the luminosity distance can be very useful when trying to measure the Hubble constant $H_0$ using \ac{GW} signals~\cite{Schutz:1986gp,Abbott:2019yzh,Soares-Santos:2019irc,Fishbach:2018gjp,Abbott:2017xzu}, and employing waveform models with \acp{HM} has been proven to be useful for this purpose~\cite{Borhanian:2020vyr}.

Furthermore, the waveform models described in this thesis have been also used to analyze all the \ac{GW} signals emitted by \acp{BBH} systems detected during the first half of the third LIGO and Virgo observing run~\cite{Abbott:2020niy,Abbott:2020tfl,Abbott:2020jks}. Employing these waveform models for this purpose is very important because their precise measurement of the binary parameters allows a better understanding of the observed population of \acp{BBH} and their formation mechanism. In addition, they have also been employed in the study of the signal GW190814~\cite{Abbott:2020khf}. In this case, the nature of the lighter compact object in the binary is unclear because its measured mass seems to be too large for a neutron star and too light for a \ac{BH}. The perculiar nature of the source of this signal was only revealed thanks to the precise measurement of the masses obtained with the waveform models described in this thesis.

There are at least two orthogonal future directions that the work of this thesis could follow. The first one involves the development of even better waveform models. A possible path for improvements is to overcome the limitation of the current models to \ac{BBH} systems in quasi-circular orbit. While there are good theoretical argoments in favour of the hypothesis that the majority of these systems feature a negligible eccentricity close to the merger, using a waveform models that allows for \acp{BBH} in generic eccentric orbits would be useful to experimentally test this thesis. The same is true for the \ac{BH} electric charge. 

The other possible direction for the future is to take advantage of the improved accuracy of the waveform models developed in this thesis for some practical applications. For example, one could exploit the more precise determination of the luminosity distance obtained with waveform models with \acp{HM} in the context of the measurement of the Hubble constant $H_0$ in binary systems composed by a neutron star and a \ac{BH}. In fact, in this case the difference between the masses of the two objects is expected to be large and the contribution of the \acp{HM} should therefore be important.


\endinput 

==> tables/allnrsims.tex <==
%\begin{tabular}{lllllll}
ID & $q$ & $\chi_1$ & $\chi_2$ & $e$ & $M\omega$ & $N_\mathrm{orb}$\\
\hline
\endfirsthead
ID & $q$ & $\chi_1$ & $\chi_2$ & $e$ & $M\omega$ & $N_\mathrm{orb}$\\
\hline
\endhead
SXS:BBH:0004 & $1.0$ & $-0.50$ & $+0.00$ & $3.7\times 10^{-4}$ & $0.01151$ & $30.2$ \\
SXS:BBH:0005 & $1.0$ & $+0.50$ & $+0.00$ & $2.5\times 10^{-4}$ & $0.01227$ & $30.2$ \\
SXS:BBH:0007 & $1.5$ & $+0.00$ & $+0.00$ & $4.2\times 10^{-4}$ & $0.01229$ & $29.1$ \\
SXS:BBH:0013 & $1.5$ & $+0.50$ & $+0.00$ & $1.4\times 10^{-4}$ & $0.01444$ & $23.8$ \\
SXS:BBH:0016 & $1.5$ & $-0.50$ & $+0.00$ & $4.2\times 10^{-4}$ & $0.01149$ & $30.7$ \\
SXS:BBH:0019 & $1.5$ & $-0.50$ & $+0.50$ & $7.6\times 10^{-5}$ & $0.01460$ & $20.4$ \\
SXS:BBH:0025 & $1.5$ & $+0.50$ & $-0.50$ & $7.6\times 10^{-5}$ & $0.01456$ & $22.4$ \\
SXS:BBH:0030 & $3.0$ & $+0.00$ & $+0.00$ & $2.0\times 10^{-3}$ & $0.01775$ & $18.2$ \\
SXS:BBH:0036 & $3.0$ & $-0.50$ & $+0.00$ & $5.1\times 10^{-4}$ & $0.01226$ & $31.7$ \\
SXS:BBH:0045 & $3.0$ & $+0.50$ & $-0.50$ & $6.4\times 10^{-4}$ & $0.01748$ & $21.0$ \\
SXS:BBH:0046 & $3.0$ & $-0.50$ & $-0.50$ & $2.6\times 10^{-4}$ & $0.01771$ & $14.4$ \\
SXS:BBH:0047 & $3.0$ & $+0.50$ & $+0.50$ & $4.7\times 10^{-4}$ & $0.01743$ & $22.7$ \\
SXS:BBH:0056 & $5.0$ & $+0.00$ & $+0.00$ & $4.9\times 10^{-4}$ & $0.01589$ & $28.8$ \\
SXS:BBH:0060 & $5.0$ & $-0.50$ & $+0.00$ & $3.4\times 10^{-3}$ & $0.01608$ & $23.2$ \\
SXS:BBH:0061 & $5.0$ & $+0.50$ & $+0.00$ & $4.2\times 10^{-3}$ & $0.01578$ & $34.5$ \\
SXS:BBH:0063 & $8.0$ & $+0.00$ & $+0.00$ & $2.8\times 10^{-4}$ & $0.01938$ & $25.8$ \\
SXS:BBH:0064 & $8.0$ & $-0.50$ & $+0.00$ & $4.9\times 10^{-4}$ & $0.01968$ & $19.2$ \\
SXS:BBH:0065 & $8.0$ & $+0.50$ & $+0.00$ & $3.7\times 10^{-3}$ & $0.01887$ & $34.0$ \\
SXS:BBH:0148 & $1.0$ & $-0.44$ & $-0.44$ & $2.0\times 10^{-5}$ & $0.01634$ & $15.5$ \\
SXS:BBH:0149 & $1.0$ & $-0.20$ & $-0.20$ & $1.8\times 10^{-4}$ & $0.01614$ & $17.1$ \\
SXS:BBH:0150 & $1.0$ & $+0.20$ & $+0.20$ & $2.9\times 10^{-4}$ & $0.01591$ & $19.8$ \\
SXS:BBH:0151 & $1.0$ & $-0.60$ & $-0.60$ & $2.5\times 10^{-4}$ & $0.01575$ & $14.5$ \\
SXS:BBH:0152 & $1.0$ & $+0.60$ & $+0.60$ & $4.3\times 10^{-4}$ & $0.01553$ & $22.6$ \\
SXS:BBH:0153 & $1.0$ & $+0.85$ & $+0.85$ & $8.3\times 10^{-4}$ & $0.01539$ & $24.5$ \\
SXS:BBH:0154 & $1.0$ & $-0.80$ & $-0.80$ & $3.3\times 10^{-4}$ & $0.01605$ & $13.2$ \\
SXS:BBH:0155 & $1.0$ & $+0.80$ & $+0.80$ & $4.7\times 10^{-4}$ & $0.01543$ & $24.1$ \\
SXS:BBH:0156 & $1.0$ & $-0.95$ & $-0.95$ & $5.4\times 10^{-4}$ & $0.01643$ & $12.4$ \\
SXS:BBH:0157 & $1.0$ & $+0.95$ & $+0.95$ & $1.4\times 10^{-4}$ & $0.01535$ & $25.2$ \\
SXS:BBH:0158 & $1.0$ & $+0.97$ & $+0.97$ & $7.9\times 10^{-4}$ & $0.01565$ & $25.3$ \\
SXS:BBH:0159 & $1.0$ & $-0.90$ & $-0.90$ & $5.6\times 10^{-4}$ & $0.01588$ & $12.7$ \\
SXS:BBH:0160 & $1.0$ & $+0.90$ & $+0.90$ & $4.2\times 10^{-4}$ & $0.01538$ & $24.8$ \\
SXS:BBH:0166 & $6.0$ & $+0.00$ & $+0.00$ & $4.4\times 10^{-5}$ & $0.01940$ & $21.6$ \\
SXS:BBH:0167 & $4.0$ & $+0.00$ & $+0.00$ & $9.9\times 10^{-5}$ & $0.02054$ & $15.6$ \\
SXS:BBH:0169 & $2.0$ & $+0.00$ & $+0.00$ & $1.2\times 10^{-4}$ & $0.01799$ & $15.7$ \\
SXS:BBH:0170 & $1.0$ & $+0.44$ & $+0.44$ & $1.3\times 10^{-4}$ & $0.00842$ & $15.5$ \\
SXS:BBH:0172 & $1.0$ & $+0.98$ & $+0.98$ & $7.8\times 10^{-4}$ & $0.01540$ & $25.4$ \\
SXS:BBH:0174 & $3.0$ & $+0.50$ & $+0.00$ & $2.9\times 10^{-4}$ & $0.01337$ & $35.5$ \\
SXS:BBH:0177 & $1.0$ & $+0.99$ & $+0.99$ & $1.3\times 10^{-3}$ & $0.01543$ & $25.4$ \\
SXS:BBH:0178 & $1.0$ & $+0.99$ & $+0.99$ & $8.6\times 10^{-4}$ & $0.01570$ & $25.4$ \\
SXS:BBH:0180 & $1.0$ & $+0.00$ & $+0.00$ & $5.1\times 10^{-5}$ & $0.01227$ & $28.2$ \\
SXS:BBH:0202 & $7.0$ & $+0.60$ & $+0.00$ & $9.0\times 10^{-5}$ & $0.01324$ & $62.1$ \\
SXS:BBH:0203 & $7.0$ & $+0.40$ & $+0.00$ & $1.4\times 10^{-5}$ & $0.01322$ & $58.5$ \\
SXS:BBH:0204 & $7.0$ & $+0.40$ & $+0.00$ & $1.7\times 10^{-4}$ & $0.01044$ & $88.4$ \\
SXS:BBH:0205 & $7.0$ & $-0.40$ & $+0.00$ & $7.0\times 10^{-5}$ & $0.01325$ & $44.9$ \\
SXS:BBH:0206 & $7.0$ & $-0.40$ & $+0.00$ & $1.6\times 10^{-4}$ & $0.01037$ & $73.2$ \\
SXS:BBH:0207 & $7.0$ & $-0.60$ & $+0.00$ & $1.7\times 10^{-4}$ & $0.01423$ & $36.1$ \\
SXS:BBH:0306 & $1.3$ & $+0.96$ & $-0.90$ & $1.5\times 10^{-3}$ & $0.02098$ & $12.6$ \\
SXS:BBH:0290 & $3.0$ & $+0.60$ & $+0.40$ & $9.0\times 10^{-5}$ & $0.01758$ & $24.2$ \\
SXS:BBH:0291 & $3.0$ & $+0.60$ & $+0.60$ & $5.0\times 10^{-5}$ & $0.01764$ & $24.5$ \\
SXS:BBH:0289 & $3.0$ & $+0.60$ & $+0.00$ & $2.3\times 10^{-4}$ & $0.01711$ & $23.8$ \\
SXS:BBH:0285 & $3.0$ & $+0.40$ & $+0.60$ & $1.6\times 10^{-4}$ & $0.01732$ & $23.8$ \\
SXS:BBH:0261 & $3.0$ & $-0.73$ & $+0.85$ & $1.0\times 10^{-4}$ & $0.01490$ & $21.5$ \\
SXS:BBH:0293 & $3.0$ & $+0.85$ & $+0.85$ & $9.0\times 10^{-5}$ & $0.01813$ & $25.6$ \\
SXS:BBH:0280 & $3.0$ & $+0.27$ & $+0.85$ & $9.7\times 10^{-5}$ & $0.01707$ & $23.6$ \\
SXS:BBH:0257 & $2.0$ & $+0.85$ & $+0.85$ & $1.1\times 10^{-4}$ & $0.01633$ & $24.8$ \\
SXS:BBH:0279 & $3.0$ & $+0.23$ & $-0.85$ & $6.0\times 10^{-5}$ & $0.01629$ & $22.6$ \\
SXS:BBH:0274 & $3.0$ & $-0.23$ & $+0.85$ & $1.6\times 10^{-4}$ & $0.01603$ & $22.4$ \\
SXS:BBH:0258 & $2.0$ & $+0.87$ & $-0.85$ & $1.8\times 10^{-4}$ & $0.01612$ & $22.8$ \\
SXS:BBH:0248 & $2.0$ & $+0.13$ & $+0.85$ & $7.0\times 10^{-5}$ & $0.01552$ & $23.2$ \\
SXS:BBH:0232 & $1.0$ & $+0.90$ & $+0.50$ & $2.8\times 10^{-4}$ & $0.01558$ & $23.9$ \\
SXS:BBH:0229 & $1.0$ & $+0.65$ & $+0.25$ & $3.1\times 10^{-4}$ & $0.01488$ & $23.1$ \\
SXS:BBH:0231 & $1.0$ & $+0.90$ & $+0.00$ & $1.0\times 10^{-4}$ & $0.01487$ & $23.1$ \\
SXS:BBH:0239 & $2.0$ & $-0.37$ & $+0.85$ & $9.1\times 10^{-5}$ & $0.01478$ & $22.2$ \\
SXS:BBH:0252 & $2.0$ & $+0.37$ & $-0.85$ & $3.8\times 10^{-4}$ & $0.01488$ & $22.5$ \\
SXS:BBH:0219 & $1.0$ & $-0.50$ & $+0.90$ & $3.3\times 10^{-4}$ & $0.01484$ & $22.4$ \\
SXS:BBH:0211 & $1.0$ & $-0.90$ & $+0.90$ & $2.6\times 10^{-4}$ & $0.01411$ & $22.3$ \\
SXS:BBH:0233 & $2.0$ & $-0.87$ & $+0.85$ & $6.0\times 10^{-5}$ & $0.01423$ & $22.0$ \\
SXS:BBH:0243 & $2.0$ & $-0.13$ & $-0.85$ & $1.8\times 10^{-4}$ & $0.01378$ & $23.3$ \\
SXS:BBH:0214 & $1.0$ & $-0.62$ & $-0.25$ & $1.9\times 10^{-4}$ & $0.01264$ & $24.4$ \\
SXS:BBH:0209 & $1.0$ & $-0.90$ & $-0.50$ & $1.7\times 10^{-4}$ & $0.01137$ & $27.0$ \\
SXS:BBH:0226 & $1.0$ & $+0.50$ & $-0.90$ & $2.4\times 10^{-4}$ & $0.01340$ & $22.9$ \\
SXS:BBH:0286 & $3.0$ & $+0.50$ & $+0.50$ & $8.0\times 10^{-5}$ & $0.01693$ & $24.1$ \\
SXS:BBH:0253 & $2.0$ & $+0.50$ & $+0.50$ & $6.7\times 10^{-5}$ & $0.01397$ & $28.8$ \\
SXS:BBH:0267 & $3.0$ & $-0.50$ & $-0.50$ & $5.6\times 10^{-5}$ & $0.01410$ & $23.4$ \\
SXS:BBH:0218 & $1.0$ & $-0.50$ & $+0.50$ & $7.8\times 10^{-5}$ & $0.01217$ & $29.1$ \\
SXS:BBH:0238 & $2.0$ & $-0.50$ & $-0.50$ & $6.9\times 10^{-5}$ & $0.01126$ & $32.0$ \\
SXS:BBH:0288 & $3.0$ & $+0.60$ & $-0.40$ & $1.9\times 10^{-4}$ & $0.01729$ & $23.5$ \\
SXS:BBH:0287 & $3.0$ & $+0.60$ & $-0.60$ & $7.0\times 10^{-5}$ & $0.01684$ & $23.5$ \\
SXS:BBH:0283 & $3.0$ & $+0.30$ & $+0.30$ & $7.6\times 10^{-5}$ & $0.01646$ & $23.5$ \\
SXS:BBH:0282 & $3.0$ & $+0.30$ & $+0.00$ & $7.5\times 10^{-5}$ & $0.01629$ & $23.3$ \\
SXS:BBH:0281 & $3.0$ & $+0.30$ & $-0.30$ & $6.7\times 10^{-5}$ & $0.01618$ & $23.2$ \\
SXS:BBH:0277 & $3.0$ & $+0.00$ & $+0.30$ & $7.0\times 10^{-5}$ & $0.01595$ & $22.9$ \\
SXS:BBH:0284 & $3.0$ & $+0.40$ & $-0.60$ & $1.5\times 10^{-4}$ & $0.01656$ & $22.8$ \\
SXS:BBH:0278 & $3.0$ & $+0.00$ & $+0.60$ & $2.1\times 10^{-4}$ & $0.01623$ & $22.8$ \\
SXS:BBH:0256 & $2.0$ & $+0.60$ & $+0.60$ & $1.0\times 10^1$ & $0.01598$ & $23.9$ \\
SXS:BBH:0230 & $1.0$ & $+0.80$ & $+0.80$ & $1.3\times 10^{-4}$ & $0.01542$ & $24.2$ \\
SXS:BBH:0255 & $2.0$ & $+0.60$ & $+0.00$ & $4.0\times 10^{-5}$ & $0.01580$ & $23.3$ \\
SXS:BBH:0276 & $3.0$ & $+0.00$ & $-0.30$ & $6.7\times 10^{-5}$ & $0.01559$ & $23.0$ \\
SXS:BBH:0251 & $2.0$ & $+0.30$ & $+0.30$ & $7.5\times 10^{-5}$ & $0.01514$ & $23.5$ \\
SXS:BBH:0250 & $2.0$ & $+0.30$ & $+0.00$ & $7.5\times 10^{-5}$ & $0.01503$ & $23.2$ \\
SXS:BBH:0271 & $3.0$ & $-0.30$ & $+0.00$ & $6.3\times 10^{-5}$ & $0.01508$ & $22.5$ \\
SXS:BBH:0249 & $2.0$ & $+0.30$ & $-0.30$ & $7.2\times 10^{-5}$ & $0.01478$ & $23.2$ \\
SXS:BBH:0275 & $3.0$ & $+0.00$ & $-0.60$ & $1.2\times 10^{-4}$ & $0.01569$ & $22.6$ \\
SXS:BBH:0254 & $2.0$ & $+0.60$ & $-0.60$ & $6.0\times 10^{-5}$ & $0.01541$ & $22.9$ \\
SXS:BBH:0269 & $3.0$ & $-0.40$ & $+0.60$ & $1.2\times 10^{-4}$ & $0.01563$ & $22.3$ \\
SXS:BBH:0225 & $1.0$ & $+0.40$ & $+0.80$ & $3.5\times 10^{-4}$ & $0.01536$ & $23.5$ \\
SXS:BBH:0270 & $3.0$ & $-0.30$ & $-0.30$ & $6.2\times 10^{-5}$ & $0.01482$ & $22.8$ \\
SXS:BBH:0245 & $2.0$ & $+0.00$ & $-0.30$ & $6.8\times 10^{-5}$ & $0.01441$ & $23.0$ \\
SXS:BBH:0242 & $2.0$ & $-0.30$ & $+0.30$ & $6.7\times 10^{-5}$ & $0.01417$ & $23.1$ \\
SXS:BBH:0223 & $1.0$ & $+0.30$ & $+0.00$ & $6.7\times 10^{-5}$ & $0.01402$ & $23.3$ \\
SXS:BBH:0241 & $2.0$ & $-0.30$ & $+0.00$ & $6.6\times 10^{-5}$ & $0.01394$ & $23.1$ \\
SXS:BBH:0240 & $2.0$ & $-0.30$ & $-0.30$ & $6.4\times 10^{-5}$ & $0.01359$ & $23.5$ \\
SXS:BBH:0222 & $1.0$ & $-0.30$ & $+0.00$ & $7.4\times 10^{-5}$ & $0.01324$ & $23.6$ \\
SXS:BBH:0228 & $1.0$ & $+0.60$ & $+0.60$ & $3.2\times 10^{-4}$ & $0.01543$ & $23.5$ \\
SXS:BBH:0247 & $2.0$ & $+0.00$ & $+0.60$ & $1.0\times 10^{-4}$ & $0.01530$ & $22.6$ \\
SXS:BBH:0263 & $3.0$ & $-0.60$ & $+0.60$ & $1.9\times 10^{-4}$ & $0.01526$ & $22.0$ \\
SXS:BBH:0266 & $3.0$ & $-0.60$ & $+0.40$ & $1.8\times 10^{-4}$ & $0.01488$ & $22.0$ \\
SXS:BBH:0227 & $1.0$ & $+0.60$ & $+0.00$ & $3.1\times 10^{-4}$ & $0.01452$ & $23.1$ \\
SXS:BBH:0221 & $1.0$ & $-0.40$ & $+0.80$ & $2.7\times 10^{-4}$ & $0.01440$ & $22.7$ \\
SXS:BBH:0237 & $2.0$ & $-0.60$ & $+0.60$ & $6.1\times 10^{-5}$ & $0.01433$ & $22.6$ \\
SXS:BBH:0244 & $2.0$ & $+0.00$ & $-0.60$ & $7.5\times 10^{-5}$ & $0.01422$ & $23.2$ \\
SXS:BBH:0217 & $1.0$ & $-0.60$ & $+0.60$ & $1.5\times 10^{-4}$ & $0.01421$ & $22.7$ \\
SXS:BBH:0215 & $1.0$ & $-0.60$ & $-0.60$ & $1.8\times 10^{-4}$ & $0.01189$ & $25.8$ \\
SXS:BBH:0262 & $3.0$ & $-0.60$ & $+0.00$ & $2.0\times 10^{-4}$ & $0.01473$ & $22.5$ \\
SXS:BBH:0213 & $1.0$ & $-0.80$ & $+0.80$ & $1.4\times 10^{-4}$ & $0.01435$ & $22.3$ \\
SXS:BBH:0265 & $3.0$ & $-0.60$ & $-0.40$ & $9.0\times 10^{-5}$ & $0.01422$ & $23.4$ \\
SXS:BBH:0264 & $3.0$ & $-0.60$ & $-0.60$ & $2.8\times 10^{-4}$ & $0.01410$ & $23.4$ \\
SXS:BBH:0224 & $1.0$ & $+0.40$ & $-0.80$ & $2.5\times 10^{-4}$ & $0.01361$ & $22.9$ \\
SXS:BBH:0236 & $2.0$ & $-0.60$ & $+0.00$ & $1.2\times 10^{-4}$ & $0.01361$ & $23.4$ \\
SXS:BBH:0216 & $1.0$ & $-0.60$ & $+0.00$ & $2.6\times 10^{-4}$ & $0.01300$ & $23.6$ \\
SXS:BBH:0235 & $2.0$ & $-0.60$ & $-0.60$ & $1.0\times 10^1$ & $0.01274$ & $25.1$ \\
SXS:BBH:0220 & $1.0$ & $-0.40$ & $-0.80$ & $1.0\times 10^{-4}$ & $0.01195$ & $25.7$ \\
SXS:BBH:0212 & $1.0$ & $-0.80$ & $-0.80$ & $2.4\times 10^{-4}$ & $0.01087$ & $28.6$ \\
SXS:BBH:0303 & $10.0$ & $+0.00$ & $+0.00$ & $5.1\times 10^{-5}$ & $0.02395$ & $19.3$ \\
SXS:BBH:0300 & $8.5$ & $+0.00$ & $+0.00$ & $5.7\times 10^{-5}$ & $0.02311$ & $18.7$ \\
SXS:BBH:0299 & $7.5$ & $+0.00$ & $+0.00$ & $5.9\times 10^{-5}$ & $0.02152$ & $20.1$ \\
SXS:BBH:0298 & $7.0$ & $+0.00$ & $+0.00$ & $6.1\times 10^{-5}$ & $0.02130$ & $19.7$ \\
SXS:BBH:0297 & $6.5$ & $+0.00$ & $+0.00$ & $6.4\times 10^{-5}$ & $0.02082$ & $19.7$ \\
SXS:BBH:0296 & $5.5$ & $+0.00$ & $+0.00$ & $5.2\times 10^{-5}$ & $0.01668$ & $27.9$ \\
SXS:BBH:0295 & $4.5$ & $+0.00$ & $+0.00$ & $5.2\times 10^{-5}$ & $0.01577$ & $27.8$ \\
SXS:BBH:0259 & $2.5$ & $+0.00$ & $+0.00$ & $5.9\times 10^{-5}$ & $0.01346$ & $28.6$ \\
SXS:BBH:0292 & $3.0$ & $+0.73$ & $-0.85$ & $1.8\times 10^{-4}$ & $0.01749$ & $23.9$ \\
SXS:BBH:0268 & $3.0$ & $-0.40$ & $-0.60$ & $1.7\times 10^{-4}$ & $0.01473$ & $22.9$ \\
SXS:BBH:0234 & $2.0$ & $-0.85$ & $-0.85$ & $1.4\times 10^{-4}$ & $0.01147$ & $27.8$ \\
SXS:BBH:0273 & $3.0$ & $-0.27$ & $-0.85$ & $2.0\times 10^{-4}$ & $0.01487$ & $22.9$ \\
SXS:BBH:0210 & $1.0$ & $-0.90$ & $+0.00$ & $1.8\times 10^{-4}$ & $0.01248$ & $24.3$ \\
SXS:BBH:0260 & $3.0$ & $-0.85$ & $-0.85$ & $3.5\times 10^{-4}$ & $0.01285$ & $25.8$ \\
SXS:BBH:0302 & $9.5$ & $+0.00$ & $+0.00$ & $6.0\times 10^{-5}$ & $0.02366$ & $19.1$ \\
SXS:BBH:0301 & $9.0$ & $+0.00$ & $+0.00$ & $5.5\times 10^{-5}$ & $0.02338$ & $18.9$ \\
SXS:BBH:0272 & $3.0$ & $-0.30$ & $+0.30$ & $6.4\times 10^{-5}$ & $0.01521$ & $22.7$ \\
SXS:BBH:0246 & $2.0$ & $+0.00$ & $+0.30$ & $7.2\times 10^{-5}$ & $0.01514$ & $22.9$ \\
%\end{tabular}


==> tables/nrsims.tex <==
\begin{tabular}{lllllll}
Id & $q$ & $\chi_1$ & $\chi_2$ & $e$ & $M\omega$ & $N_\mathrm{orb}$\\
\hline
SXS:BBH:0610 & $1.2$ & $-0.50$ & $-0.50$ & $7.4\times 10^{-5}$ & $0.01872$ & $12.1$ \\
SXS:BBH:0611 & $1.4$ & $-0.50$ & $+0.50$ & $6.0\times 10^{-4}$ & $0.02033$ & $12.5$ \\
SXS:BBH:0612 & $1.6$ & $+0.50$ & $-0.50$ & $3.7\times 10^{-4}$ & $0.02156$ & $12.8$ \\
SXS:BBH:0613 & $1.8$ & $+0.50$ & $+0.50$ & $1.8\times 10^{-4}$ & $0.02383$ & $13.1$ \\
SXS:BBH:0614 & $2.0$ & $+0.75$ & $-0.50$ & $6.7\times 10^{-4}$ & $0.02355$ & $13.1$ \\
SXS:BBH:0615 & $2.0$ & $+0.75$ & $+0.00$ & $7.0\times 10^{-4}$ & $0.02401$ & $13.3$ \\
SXS:BBH:0616 & $2.0$ & $+0.75$ & $+0.50$ & $8.0\times 10^{-4}$ & $0.02475$ & $13.3$ \\
SXS:BBH:0617 & $2.0$ & $+0.50$ & $+0.75$ & $7.8\times 10^{-4}$ & $0.02342$ & $13.1$ \\
SXS:BBH:0618 & $2.0$ & $+0.80$ & $+0.80$ & $5.9\times 10^{-4}$ & $0.02578$ & $13.4$ \\
SXS:BBH:0619 & $2.0$ & $+0.90$ & $+0.90$ & $2.9\times 10^{-4}$ & $0.02520$ & $13.5$ \\
SXS:BBH:0620 & $5.0$ & $-0.80$ & $+0.00$ & $1.7\times 10^{-4}$ & $0.02551$ & $8.1$ \\
SXS:BBH:0621 & $7.0$ & $-0.80$ & $+0.00$ & $4.8\times 10^{-4}$ & $0.02828$ & $7.2$ \\
SXS:BBH:0622 & $8.0$ & $-0.90$ & $+0.00$ & $1.1\times 10^{-3}$ & $0.01559$ & $28.0$ \\
\hline
ET:AEI:0001 & $5.0$ & $+0.80$ & $+0.00$ & $9.2\times 10^{-4}$ & $0.03077$ & $10.5$ \\
ET:AEI:0002 & $7.0$ & $+0.80$ & $+0.00$ & $6.1\times 10^{-4}$ & $0.03503$ & $10.4$ \\
ET:AEI:0003 & $8.0$ & $+0.85$ & $+0.85$ & $1.2\times 10^{-2}$ & $0.04099$ & $7.4$ \\
\end{tabular}


==> tables/sets/bam.tex <==
ID & $q$ & $\chi_1$ & $\chi_2$ & $e$ & $M\omega_{22}$ & $N_\mathrm{orb}$\\
\hline
BAMq8s85s85 & $8.0$ & $+0.85$ & $+0.85$ & $9.1\times 10^{-3}$ & $0.05476$ & $7.9$ \\

